To Model or to Intervene: A Comparison of Counterfactual and Online Learning to Rank from User Interactions

Learning to Rank (LTR) from user interactions is challenging as user feedback often contains high levels of bias and noise. At the moment, two methodologies for dealing with bias prevail in the field of LTR: counterfactual methods that learn from historical data and model user behavior to deal with biases; and online methods that perform interventions to deal with bias but use no explicit user models. For practitioners the decision between either methodology is very important because of its direct impact on end users. Nevertheless, there has never been a direct comparison between these two approaches to unbiased LTR. In this study we provide the first benchmarking of both counterfactual and online LTR methods under different experimental conditions. Our results show that the choice between the methodologies is consequential and depends on the presence of selection bias, and the degree of position bias and interaction noise. In settings with little bias or noise counterfactual methods can obtain the highest ranking performance; however, in other circumstances their optimization can be detrimental to the user experience. Conversely, online methods are very robust to bias and noise but require control over the displayed rankings. Our findings confirm and contradict existing expectations on the impact of model-based and intervention-based methods in LTR, and allow practitioners to make an informed decision between the two methodologies.

==> tables/linear-models-offline.tex <==
% !TEX root = ../thesis.tex
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill} } l  l l l l l  }
\toprule
 & \multicolumn{1}{l}{ \small \textbf{MQ2007}}  & \multicolumn{1}{l}{ \small \textbf{MQ2008}}  & \multicolumn{1}{l}{ \small \textbf{MSLR-WEB10k}}  & \multicolumn{1}{l}{ \small \textbf{Yahoo}}  & \multicolumn{1}{l}{ \small \textbf{Istella}} \\
\midrule
& \multicolumn{5}{c}{\textit{perfect}} \\
\midrule
\acs{DBGD} & {\small 0.417 {\tiny( 0.02)}} & {\small 0.492 {\tiny( 0.04)}} & {\small 0.320 {\tiny( 0.01)}} & {\small 0.658 {\tiny( 0.01)}} & {\small 0.447 {\tiny( 0.01)}} \\
\acs{MGD} & {\small 0.426 {\tiny( 0.02)}} & {\small 0.499 {\tiny( 0.04)}} & {\small 0.323 {\tiny( 0.00)}} & {\small 0.688 {\tiny( 0.00)}} & {\small 0.497 {\tiny( 0.00)}} \\
Pairwise-Baseline & {\small 0.411 {\tiny( 0.03)}} & {\small 0.496 {\tiny( 0.04)}} & {\small 0.332 {\tiny( 0.04)}} & {\small 0.631 {\tiny( 0.04)}} & {\small 0.536 {\tiny( 0.02)}} \\
\acs{\OurMethod}-linear & \textbf {\small 0.439 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.505 {\tiny( 0.04)}} {\tiny \enkelop} \hphantom{\tiny \dubbelneer} \hphantom{\tiny \dubbelneer} & \textbf {\small 0.414 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.711 {\tiny( 0.00)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.571 {\tiny( 0.00)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 0.438 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.505 {\tiny( 0.04)}} {\tiny \enkelop} \hphantom{\tiny \dubbelneer} \hphantom{\tiny \dubbelneer} & \textbf {\small 0.414 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.707 {\tiny( 0.00)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.569 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\midrule
& \multicolumn{5}{c}{\textit{navigational}} \\
\midrule
\acs{DBGD} & {\small 0.399 {\tiny( 0.02)}} & {\small 0.481 {\tiny( 0.04)}} & {\small 0.309 {\tiny( 0.01)}} & {\small 0.637 {\tiny( 0.02)}} & {\small 0.400 {\tiny( 0.02)}} \\
\acs{MGD} & {\small 0.366 {\tiny( 0.02)}} & {\small 0.476 {\tiny( 0.03)}} & {\small 0.311 {\tiny( 0.00)}} & {\small 0.680 {\tiny( 0.02)}} & {\small 0.404 {\tiny( 0.00)}} \\
Pairwise-Baseline & {\small 0.403 {\tiny( 0.03)}} & {\small 0.481 {\tiny( 0.04)}} & {\small 0.322 {\tiny( 0.04)}} & {\small 0.612 {\tiny( 0.03)}} & {\small 0.423 {\tiny( 0.07)}} \\
\acs{\OurMethod}-linear & \textbf {\small 0.426 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.502 {\tiny( 0.04)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.373 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \bf {\small 0.699 {\tiny( 0.00)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.538 {\tiny( 0.00)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 0.419 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.499 {\tiny( 0.04)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.331 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \enkelop} & {\small 0.697 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.528 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\midrule
& \multicolumn{5}{c}{\textit{informational}} \\
\midrule
\acs{DBGD} & {\small 0.357 {\tiny( 0.03)}} & {\small 0.454 {\tiny( 0.04)}} & {\small 0.288 {\tiny( 0.02)}} & {\small 0.592 {\tiny( 0.04)}} & {\small 0.361 {\tiny( 0.03)}} \\
\acs{MGD} & {\small 0.349 {\tiny( 0.02)}} & {\small 0.465 {\tiny( 0.04)}} & {\small 0.307 {\tiny( 0.00)}} & {\small 0.637 {\tiny( 0.06)}} & {\small 0.388 {\tiny( 0.00)}} \\
Pairwise-Baseline & {\small 0.338 {\tiny( 0.05)}} & {\small 0.404 {\tiny( 0.06)}} & {\small 0.252 {\tiny( 0.05)}} & {\small 0.579 {\tiny( 0.04)}} & {\small 0.131 {\tiny( 0.09)}} \\
\acs{\OurMethod}-linear & \textbf {\small 0.422 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.496 {\tiny( 0.04)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.361 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \bf {\small 0.686 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.530 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 0.415 {\tiny( 0.02)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 0.496 {\tiny( 0.04)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.333 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \bf {\small 0.686 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 0.523 {\tiny( 0.01)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\bottomrule
\end{tabular*}


==> tables/linear-models-online.tex <==
% !TEX root = ../thesis.tex
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill} } l  l l l l l  }
\toprule
 & \multicolumn{1}{l}{ \small \textbf{MQ2007}}  & \multicolumn{1}{l}{ \small \textbf{MQ2008}}  & \multicolumn{1}{l}{ \small \textbf{MSLR-WEB10k}}  & \multicolumn{1}{l}{ \small \textbf{Yahoo}}  & \multicolumn{1}{l}{ \small \textbf{Istella}} \\
\midrule
& \multicolumn{5}{c}{\textit{perfect}} \\
\midrule
\acs{DBGD} & {\small 671.9 {\tiny( 23.3)}} & {\small 843.8 {\tiny( 23.3)}} & {\small 532.1 {\tiny( 16.0)}} & {\small 1151.6 {\tiny( 28.7)}} & {\small 601.5 {\tiny( 19.6)}} \\
\acs{MGD} & {\small 690.4 {\tiny( 12.6)}} & {\small 859.1 {\tiny( 20.0)}} & {\small 559.3 {\tiny( 7.0)}} & {\small 1202.2 {\tiny( 11.2)}} & {\small 686.1 {\tiny( 8.4)}} \\
Pairwise-Baseline & {\small 594.6 {\tiny( 10.2)}} & {\small 747.9 {\tiny( 18.5)}} & {\small 458.2 {\tiny( 6.1)}} & {\small 1115.6 {\tiny( 9.9)}} & {\small 342.4 {\tiny( 7.3)}} \\
\acs{\OurMethod}-linear & \textbf {\small 778.6 {\tiny( 13.2)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 947.4 {\tiny( 22.2)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 659.1 {\tiny( 12.7)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 1305.2 {\tiny( 8.3)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 910.5 {\tiny( 10.1)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 691.3 {\tiny( 12.1)}} {\tiny \dubbelop} \hphantom{\tiny \dubbelneer} {\tiny \dubbelop} & {\small 890.2 {\tiny( 22.1)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & {\small 558.0 {\tiny( 12.2)}} {\tiny \dubbelop} \hphantom{\tiny \dubbelneer} {\tiny \dubbelop} & {\small 1133.4 {\tiny( 9.9)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelop} & {\small 698.7 {\tiny( 21.7)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\midrule
& \multicolumn{5}{c}{\textit{navigational}} \\
\midrule
\acs{DBGD} & {\small 637.5 {\tiny( 27.1)}} & {\small 815.0 {\tiny( 25.4)}} & {\small 508.4 {\tiny( 23.4)}} & {\small 1130.0 {\tiny( 29.1)}} & {\small 549.8 {\tiny( 29.7)}} \\
\acs{MGD} & {\small 635.5 {\tiny( 13.0)}} & {\small 822.3 {\tiny( 18.5)}} & {\small 537.9 {\tiny( 7.9)}} & {\small 1178.4 {\tiny( 23.0)}} & {\small 607.4 {\tiny( 9.8)}} \\
Pairwise-Baseline & {\small 585.7 {\tiny( 10.9)}} & {\small 737.7 {\tiny( 16.8)}} & {\small 442.2 {\tiny( 9.6)}} & {\small 1106.0 {\tiny( 8.1)}} & {\small 272.6 {\tiny( 12.2)}} \\
\acs{\OurMethod}-linear& \textbf {\small 671.8 {\tiny( 14.1)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 879.7 {\tiny( 21.2)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 554.0 {\tiny( 12.6)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 1287.6 {\tiny( 20.1)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 632.7 {\tiny( 21.9)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 528.7 {\tiny( 9.6)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelneer} & {\small 734.3 {\tiny( 19.4)}} {\tiny \dubbelneer} {\tiny \dubbelneer} \hphantom{\tiny \dubbelneer} & {\small 411.5 {\tiny( 8.6)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelneer} & {\small 1131.9 {\tiny( 13.9)}} \hphantom{\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelop} & {\small 225.5 {\tiny( 23.7)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelneer} \\
\midrule
& \multicolumn{5}{c}{\textit{informational}} \\
\midrule
\acs{DBGD} & {\small 581.4 {\tiny( 40.1)}} & {\small 762.3 {\tiny( 43.6)}} & {\small 473.6 {\tiny( 34.6)}} & {\small 1104.0 {\tiny( 36.3)}} & {\small 433.5 {\tiny( 61.4)}} \\
\acs{MGD} & {\small 620.4 {\tiny( 17.2)}} & {\small 815.0 {\tiny( 36.6)}} & {\small 538.7 {\tiny( 8.0)}} & {\small 1145.9 {\tiny( 47.7)}} & {\small 595.5 {\tiny( 10.9)}} \\
Pairwise-Baseline & {\small 551.0 {\tiny( 9.7)}} & {\small 708.0 {\tiny( 17.9)}} & {\small 408.8 {\tiny( 7.5)}} & {\small 1090.4 {\tiny( 8.5)}} & {\small 122.9 {\tiny( 6.9)}} \\
\acs{\OurMethod}-linear & \textbf {\small 681.4 {\tiny( 28.7)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 889.4 {\tiny( 24.6)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 554.3 {\tiny( 32.5)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 1262.3 {\tiny( 38.4)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} & \textbf {\small 659.8 {\tiny( 95.8)}} {\tiny \dubbelop} {\tiny \dubbelop} {\tiny \dubbelop} \\
\acs{\OurMethod}-neural & {\small 551.1 {\tiny( 13.6)}} {\tiny \dubbelneer} {\tiny \dubbelneer} \hphantom{\tiny \dubbelneer} & {\small 765.3 {\tiny( 22.9)}} \hphantom{\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelop} & {\small 435.7 {\tiny( 13.1)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelop} & {\small 1139.0 {\tiny( 15.9)}} {\tiny \dubbelop} \hphantom{\tiny \dubbelneer} {\tiny \dubbelop} & {\small 311.0 {\tiny( 52.3)}} {\tiny \dubbelneer} {\tiny \dubbelneer} {\tiny \dubbelop} \\
\bottomrule
\end{tabular*}

